Graded Unitarity in the SCFT/VOA Correspondence

Vertex algebras that arise from four-dimensional, $\mathcal{N}=2$ superconformal field theories inherit a collection of novel structural properties from their four-dimensional ancestors. Crucially, when the parent SCFT is unitary, the corresponding vertex algebra is not unitary in the conventional sense. In this paper, we motivate and define a generalized notion of unitarity for vertex algebras that we call \emph{graded unitarity}, and which captures the consequences of four-dimensional unitarity under this correspondence. We also take the first steps towards a classification program for graded-unitary vertex algebras whose underlying vertex algebras are Virasoro or affine Kac--Moody vertex algebras. Remarkably, under certain natural assumptions about the $\mathfrak{R}$-filtration for these vertex algebras, we show that only the $(2,p)$ central charges for Virasoro VOAs and boundary admissible levels for $\mathfrak{sl}_2$ and $\mathfrak{sl}_3$ Kac--Moody vertex algebras can possibly be compatible with graded unitarity. These are precisely the cases of these vertex algebras that are known to arise from four dimensions.

==> topmatter.tex <==
%!TEX Root = ./main.tex

\RequirePackage{pdf14}
\RequirePackage{fix-cm}
\usepackage{./aux/jheppub}

\usepackage{graphicx,adjustbox}
\usepackage{amsfonts,amsmath,amssymb,amsthm}
\usepackage{tikz,tikz-cd}
\usetikzlibrary{positioning}
\usepackage{verbatim}
\usepackage[parfill]{parskip}
\usepackage{array,setspace,mathrsfs,yfonts,dsfont,amscd,euscript}
\usepackage{relsize,suffix,mathtools,cancel,bm,bbm}

\setcounter{tocdepth}{2}


%Theorem environments
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{corr}[thm]{Corollary}
\newtheorem{rem}[thm]{Remark}

\newtheorem*{sthm}{Theorem}
